Transformers in Remote Sensing: A Survey

Deep learning-based algorithms have seen a massive popularity in different areas of remote sensing image analysis over the past decade. Recently, transformers-based architectures, originally introduced in natural language processing, have pervaded computer vision field where the self-attention mechanism has been utilized as a replacement to the popular convolution operator for capturing long-range dependencies. Inspired by recent advances in computer vision, remote sensing community has also witnessed an increased exploration of vision transformers for a diverse set of tasks. Although a number of surveys have focused on transformers in computer vision in general, to the best of our knowledge we are the first to present a systematic review of recent advances based on transformers in remote sensing. Our survey covers more than 60 recent transformers-based methods for different remote sensing problems in sub-areas of remote sensing: very high-resolution (VHR), hyperspectral (HSI) and synthetic aperture radar (SAR) imagery. We conclude the survey by discussing different challenges and open issues of transformers in remote sensing. Additionally, we intend to frequently update and maintain the latest transformers in remote sensing papers with their respective code at: https://github.com/VIROBO-15/Transformer-in-Remote-Sensing

==> Transformers in remote sensing-a survey/Table1.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}


\begin{table*}[h]
\renewcommand{\arraystretch}{1.5}
	\centering
	
	\caption{Overview of transformers-based approaches in VHR remote sensing imaging. Here, we highlight transformers-based methods for different VHR remote sensing tasks.} 	\label{tab:Main_table}
	{\resizebox*{\textwidth}{\textheight}{%
	%\resizebox{!}{.40\paperheight}{%
	%\resizebox{\textwidth}{!}{
	%\begin{longtable}{|*{3}{>{\centering\arraybackslash}p{3cm}|}}
		\begin{tabular}{V{3}l|c|c|c|P{7cm}V{3}} \hlineB{3}
		\rowcolor{mygray} \multicolumn{5}{|c|}{\textbf{Transformers in Very-High Resolution (VHR) Satellite Imagery}} \\ \hlineB{2}
		\rowcolor{mygray}	\textbf{Method}& \textbf{Task}& \textbf{Datasets}& \textbf{Metrics}& \textbf{Highlights} \\\hlineB{2}
			
			%---------



			 V16-21K \cite{bazi2021vision} &Classification&\makecell{Merced\cite{yang2010bag},\\ AID\cite{xia2017aid},\\ Optimal31\cite{wang2018scene},\\ NWPU\cite{cheng2017remote}}&Overall classification accuracy& Explores vision transformers along with combination of data augmentation techniques for boosting accuracy.\\\hline
			 
			 TRS \cite{zhang2021trs} &Classification&\makecell{Merced\cite{yang2010bag},\\ AID\cite{xia2017aid},\\ Optimal31\cite{wang2018scene},\\ NWPU\cite{cheng2017remote}}&Overall classification accuracy&Integrates transformers into CNNs by replacing the last three ResNet bottlenecks with encoders having multi-head self-attention bottleneck.\\\hline
			 
			 TSTNet\cite{hao2022two}&Classification&\makecell{Merced\cite{yang2010bag},\\ AID\cite{xia2017aid},\\ NWPU\cite{cheng2017remote}}&\makecell{Overall classification accuracy}&A Swin transformer based two-stream architecture that uses both deep features from the image and edge features from edge stream.\\\hline
			 
			 
			 CTNet\cite{deng2021cnns}&Classification &\makecell{AID\cite{xia2017aid},\\ NWPU\cite{cheng2017remote}}&Overall classification accuracy&Comprises a ViT stream that mines semantic features and the CNN stream which captures local structural features.\\\hline
			 
			 
			 HHTL\cite{ma2022homo}&Classification &\makecell{Merced\cite{yang2010bag},\\ AID\cite{xia2017aid},\\ RSSDIVCS\cite{li2021learning},\\ NWPU\cite{cheng2017remote}}&\makecell{Overall classification accuracy}&Explores integrating heterogenous non-overlapping patches and homogenous patches obtained using superpixel segmentation.\\\hline
			 
			 RSP \cite{Wang2022empirical}&Classification, Segmentation, Detection &\makecell{MillionAID\cite{MillionAID},\\ Potsdam \cite{Potsdam},\\ iSAID\cite{waqas2019isaid},\\ HRSC2016 \cite{liu2017high},\\ DOTA\cite{xia2018dota},\\ CCD\cite{lebedev2018change},\\ LEVIR\cite{chen2020spatial}}&\makecell{Overall classification accuracy,\\ mAP,\\ F1 score}&Investigates pre-training transformers on a large-scale remote sensing dataset.\\\hline
%----------------------------------------------------------%			 
			 SAIEC \cite{xu2021improved}&Detection, Segmentation &\makecell{DIOR\cite{li2020object},\\ HRRSD\cite{zhang2019hierarchical},\\ NWPU VHR-10\cite{cheng2016learning}}&\makecell{mAP}&Introduces a local perception Swin transformer backbone that aims to combine the merits of transformers and CNNs for improving the local perception capabilities.\\\hline
			 
			 T-TRD-DA \cite{li2022transformer}&Detection &\makecell{DIOR\cite{li2020object},\\ NWPU VHR-10\cite{cheng2016learning}}
			 &\makecell{mAP}& Proposes a transformers-based detector utilizing a pre-trained CNN for feature extraction and multiple-layer transformers for multi-scale feature aggregation at global spatial positions.  \\\hline
             
			GANsformer \cite{zhang2022gansformer}&Detection &\makecell{DIOR\cite{li2020object},\\ NWPU VHR-10\cite{cheng2016learning}}
			 &\makecell{mAP}& Introduces an efficient transformer, with reduced parameters, as a branch network to capture global features along with a generative model to expand the input image ahead of backbone.\\\hline
			 
			ADT-Det \cite{ADTDet}&Detection &\makecell{DIOR\cite{li2020object},\\ HRSC2016 \cite{liu2017high}}
			&\makecell{mAP}& Introduces a RetineNet-based framework with a feature pyramid transformer integrated between the backbone and post-processing network for generating multi-scale semantic features.\\\hline
			 
			 			 
            PointRCNN \cite{PointRCNN}&Detection &\makecell{DOTA\cite{xia2018dota},\\ HRSC2016 \cite{liu2017high} }
			&\makecell{mAP}& Introduces a two-stage angle-free dectection framework which is also evaluated using the transformers-based Swin backbone.\\\hline


            HybridNetwork22 \cite{HybridNetwork22}&Detection &\makecell{DOTA\cite{xia2018dota},\\ UCAS-AOD\cite{zhu2015orientation},\\ VEDAI\cite{razakarivony2016vehicle}}&\makecell{mAP}& Integrates multi-scale global and local information from transformers and CNNs through an adaptive feature fusion network.\\\hline
			 
            Oriented RepPoints \cite{li2021oriented}&Detection &\makecell{DOTA\cite{xia2018dota},\\ UCAS-AOD\cite{zhu2015orientation},\\ HRSC2016 \cite{liu2017high}}
			&\makecell{mAP}& Proposes an anchor-free detector learns flexible adaptive points as representations through a quality assessment and sample assignment scheme.\\\hline
			 
			 
            O$^{2}$DETR \cite{MaOrientedDetr}&Detection &\makecell{DOTA\cite{xia2018dota},\\ SKU110K-R\cite{pan2020dynamic},\\ HRSC2016 \cite{liu2017high}}
			&\makecell{mAP}&Extends the standard DETR for oriented detection by introducing an encoder employing depthwise separable convolution. \\\hline
			
			
			 
            AO2DETR \cite{AO2DETR}&Detection &\makecell{DOTA\cite{xia2018dota}}
			&\makecell{mAP}&Introduces a DETR-based detector with oriented proposal generation scheme, a refine module to compute rotation-invariant features and a rotation-aware matching loss for performing the matching process for direct set predictions. \\\hline
			
		RBox \cite{Tangcvpr22}&Detection &\makecell{SynthText\cite{gupta2016synthetic},\\ ICDAR 2015 (IC15)\cite{karatzas2015icdar},\\ MLT-2017 (MLT17)\cite{nayef2017icdar2017},\\ MSRA-TD500\cite{yao2012detecting},\\ MTWI\cite{he2018icpr2018},\\ Total-Text\cite{ch2017total},\\ CTW1500\cite{yuliang2017detecting}}
			&\makecell{mAP}&Proposes a framework employing transformers to model the relationship of sampled features for better grouping and box prediction without requiring post-processing operation.\\\hline
			
			Rodformer \cite{Rodformer}&Detection&\makecell{DOTA\cite{xia2018dota}}
			&\makecell{mAP}&A hybrid detection architecture integrating the local characteristics of depth-separable convolutions with the global characteristics of MLP.\\\hline
%----------------------------------------------------------%

			CD-Trans \cite{ChenCDTGRS}&Change Detection&\makecell{WHU\cite{ji2018fully},\\ LEVIR\cite{chen2020spatial},\\ DSIFN\cite{zhang2020deeply}}
			&\makecell{F1 score} &Introduces a bi-temporal image transformer designed to model the spatio-temporal contextual information. The encoder captures context in token-based space-time,  which are then fed to decoder where feature refinement is performed in the pixel-space. \\\hline
			
			
			
        %    UVACD \cite{Guanghui22RS}&Change Detection &\makecell{WHU\cite{ji2018fully},LEVIR\cite{chen2020spatial}}	&\makecell{F1 score}&Proposes an approach where semantic features are extracted via CNN backbone and transformers are employed to produce change features through encoding temporal information interaction. \\\hline
			
        %    TransUNetCD \cite{li2022transunetcd}&Change Detection &\makecell{WHU\cite{ji2018fully}, LEVIR\cite{chen2020spatial}, CCD\cite{lebedev2018change}, DSIFN\cite{zhang2020deeply}, OSCD\cite{daudt2018urban}, S2Looking\cite{shen2021s2looking}}
		%	&\makecell{F1 score}&Introduces a framework integrating merits of transformers and UNet through capturing enriched contextualized features which are upsampled and fused with multi-scale features to generate global-local features. \\\hline
			
		%	Hybrid-TransCD \cite{HybridTransCD}&Change Detection &\makecell{LEVIR\cite{chen2020spatial}, SYSU-CD\cite{shi2021deeply}}
		%	&\makecell{F1 score}&Introduces a multi-scale transformer that encodes both fine-grained and large object features through heterogeneous tokens via multiple receptive fields.\\\hline
			
			
%----------------------------------------------------------------%
		%	 CCTNet \cite{wang2022cctnet}&Segmentation &\makecell{Barley Remote Sensing Dataset \tablefootnote{Dataset is available at: \url{https://tianchi.aliyun.com/dataset/dataDetail?dataId=74952}}}&\makecell{F1 score, Overall accuracy}& Proposes a hybrid CNN-transformers framework to combine local details and global conextual information for crop segmentation. \\\hline
			 
		%	 STransFuse \cite{9573374}&Segmentation &\makecell{Potsdam\tablefootnotemark[\ref{Potsdam}], Vaihingen\tablefootnotemark[\ref{Vaihingen}] }&\makecell{F1 score, Overall accuracy}& Introduces a framework that encodes both coarse-grained as well as fine-grained features at multiple scales which are fused using self-attentive mechanism. \\\hline
			 
		%	 Trans-CNN \cite{9686732}&Segmentation&\makecell{Potsdam\tablefootnotemark[\ref{Potsdam}, Vaihingen\tablefootnotemark[\ref{Vaihingen} }&\makecell{F1 score, Overall accuracy}& Introduces a framework with a Swin transformer backbone to capture long-range dependencies and a U-shaped decoder with depth-wise separable convolution to encode local details. \\\hline
			 
			% Xu \etal\cite{xu2021improved}&Segmentation&\makecell{DIOR\cite{li2020object}, HRRSD\cite{zhang2019hierarchical},  NWPU VHR-10\cite{cheng2016learning}}&\makecell{F1 score, Overall accuracy}&A local perception Swin transformer backbone, taking advantage of both CNNs and transformers.\\\hline
			 
	%	SwinTF \cite{panboonyuen2021transformer}&Segmentation &\makecell{Vaihingen\tablefootnotemark[\ref{Vaihingen}], Thailand North Landsat-8 corpus (private), Thailand Isan Landsat-8 corpus (private)}&\makecell{F1 score, Overall accuracy}&Introduces a framework with pre-trained Swin backbone along with a U-Net, feature pyramid network and a pyramid scene parsing network for segmentation. \\\hline
			 
	%		Efficient-T \cite{xu2021efficient}&Segmentation &\makecell{Potsdam\tablefootnotemark[\ref{Potsdam}, Vaihingen\tablefootnotemark[\ref{Vaihingen} }&\makecell{F1 score, Overall accuracy}& Proposes a light-weight framework consisting of an implicit edge enhancement scheme along with a Swin transformers.\\\hline
			 
%--------------------------------------------------------
	%		 STT \cite{chen2021building}&Building Extraction &\makecell{WHU\cite{ji2018fully}, INRIA\cite{maggiori2017can}}&\makecell{IoU, Overall accuracy, F1 score}&Introduces a transformers framework to learn long-range dependencies both in the spatial and channel direction. \\\hline
			 
	%		 STEB-UNet \cite{xiao2022swin}&Building Extraction &\makecell{WHU\cite{ji2018fully}, Massachusetts\cite{maggiori2017can}}&\makecell{IoU, F1 score}&Introduces a transformers framework capturing semantic information from multi-scale features which are further fused to local features. \\\hline
			 
	%		 BuildFormer \cite{wang2022buildformer}&Building Extraction &\makecell{WHU\cite{ji2018fully}, Massachusetts\cite{maggiori2017can},
	%		 INRIA\cite{maggiori2017can}}& \makecell{IoU, F1 score}&A Introduces an architecture consisitng of a window-based linear attention and a convolutional MLP.\\\hline
			 
	%		 T-Trans \cite{qiu2022transferring}&Building Extraction &\makecell{Massachusetts\cite{maggiori2017can}
			 %,INRIA\cite{maggiori2017can}}&\makecell{IoU, F1 score}& Explores the task of generalizability of building extraction models to different areas and introduces a transfer learning method to fine-tune models from one area to a subset of another unseen area.  \\\hline
			 
 %-------------------------------------------------%
 
	%	    TRL \cite{shen2020remote}&\makecell{Image Captioning} &\makecell{RSICD\cite{lu2017exploring}, UCM-captions \tablefootnote{\label{UCM}Dataset is available: \url{https://mega.nz/folder/wCpSzSoS#RXzIlrv--TDt3ENZdKN8JA}}, Sydney-Caption\tablefootnote{\label{sydney}Dataset is available at: \url{https://mega.nz/folder/pG4yTYYA#4c4buNFLibr\\yZnlujsrwEQ}}}
	%		&\makecell{BLEU, ROUGE, METEOR, CIDEr}&Proposes an approach adapting transformers by integrating residual connections, dropout and adatpive feature fusion for remote sensing image caption generation. \\\hline
			
	%		MLAT\cite{liu2022remote}&\makecell{Image Captioning} &\makecell{RSICD\cite{lu2017exploring}, UCM-captions\tablefootnotemark[\ref{UCM}], Sydney-Caption\tablefootnotemark[\ref{sydney}]}
	%		&\makecell{BLEU, ROUGE, METEOR, CIDEr}&Introduces an architecture where multi-scale features from CNN layers are extracted in encoder and a multi-layer aggregated transformer in the decoder uses those features for sentence generation. \\\hline
			
	%		Ren \etal\cite{ren2022mask}&\makecell{Image Captioning} &\makecell{RSICD\cite{lu2017exploring}, UCM-captions\tablefootnotemark[\ref{UCM}], Sydney-Caption\tablefootnotemark[\ref{sydney}]}
	%		&\makecell{BLEU, ROUGE, METEOR, CIDEr}&Proposes a topic token-based mask transformers  with the topic token being integrated into encoder while serving as prior in decoder for capturing global semantic relationships.\\\hline
			
% 			\cite{Ren22RS}&\makecell{Image Captioning} &\makecell{RSICD\cite{lu2017exploring} \\UCM-captions \cite{yang2010bag,qu2016deep}\\Sydney-Caption\cite{zhang2014saliency,qu2016deep}}
% 			&\makecell{BLEU\\ROUGE\\METEOR\\CIDEr\\Self-CIDEr}&Introduces a transformer-based multi-stage enhancement structure.\\\hline

%-------------------------------------------------%
	%		TR-MISR \cite{an2022tr}&\makecell{Image Super Resolution}&\makecell{RSICD\cite{lu2017exploring}, UCM-captions\tablefootnotemark[\ref{UCM}], PROBA-V\cite{martens2019super}}
	%		&\makecell{cPSNR, cSSIM}&Introduces a transformers-based architecture with an encoder having residual blocks, a fusion module along with a super-pixel convolution-based decoder for multi-image super-resolution. \\\hline
			
	%		MSE-Net \cite{lei2021transformer}&\makecell{Image Super Resolution}&\makecell{UCMerced \tablefootnote{\label{ucmerced}Dataset is available at: \url{http://vision.ucmerced.edu/datasets/landuse.html}}, AID\cite{xia2017aid}}
	%		&\makecell{cPSNR, cSSIM}&Proposes a multi-stage enchancement framework to utilize features from different stages and further integrating them with standard super-resolution technique for combining multi-resolution low as well as high-dimension feature representations. \\\hline
			
	%	SRT \cite{ye2021super}&\makecell{Image Super Resolution}&\makecell{UCMerced\tablefootnotemark[\ref{ucmerced}]}
	%		&\makecell{cPSNR, cSSIM}&Introduces a hybrid framework that integrates local features from CNNs and global features from transformers. \\\hline

		    
		\end{tabular}
		}  
	%	\caption{An overview of transformers-based approaches in VHR remote sensing imaging. Here, we highlight methods for different VHR remote sensing tasks.} 
                % These are some of the datasets used for VHR imagery, Merced\cite{yang2010bag}, Optimal31\cite{wang2018scene}, NWPU\cite{cheng2017remote}, RSSDIVCS\cite{li2021learning}, MillionAID\cite{MillionAID}, iSAID\cite{waqas2019isaid}, HRSC2016 \cite{liu2017high}, CCD\cite{lebedev2018change}, LEVIR\cite{chen2020spatial}, DIOR\cite{li2020object}, HRRSD\cite{zhang2019hierarchical}, }
}
\end{table*}
%----------------------------------------------------------%
% \begin{table*}[t!]
% \renewcommand{\arraystretch}{1.5}
% 	\centering
% 	{\resizebox*{\textwidth}{\textheight}{%
% 	%\resizebox{!}{.40\paperheight}{%
% 	%\resizebox{\textwidth}{!}{
% 	%\begin{longtable}{|*{3}{>{\centering\arraybackslash}p{3cm}|}}
% 	\begin{tabular}{V{3}l|c|c|c|P{7cm}V{3}} \hlineB{3}
		
% 		\rowcolor{mygray}	\textbf{Method}& \textbf{Task}& \textbf{Datasets}& \textbf{Metrics}& \textbf{Highlights} \\\hlineB{2}
		
% 			 CCTnet\cite{wang2022cctnet}&Segmentation &\makecell{Barley Remote Sensing Dataset \tablefootnote{Dataset is available at: https://tianchi.aliyun.com/dataset/dataDetail?dataId=74952}}&\makecell{Precision \\ Recall \\ F1 \\ OA \\ mIoU}&Introduces a model combining the advantages of CNNs in local modeling and Transformer in global modeling.\\\hline
			 
% 			 STransFuse\cite{9573374}&Segmentation &\makecell{Potsdam \cite{isprs20192d} \\Vaihingen\cite{rottensteinerinternational}}&\makecell{F1 \\ OA \\ mIoU}&Introduces a model by fusing Swin Transformer and CNN, resulting in a two-branch model that combines the advantages of Transformer network and CNN.\\\hline
			 
% 			 \cite{9686732}&Segmentation&\makecell{Potsdam \cite{isprs20192d} \\Vaihingen\cite{rottensteinerinternational}}&\makecell{F1 \\ OA}&A CNN and transformer hybrid deep neural network for VHR remote sensing images semantic segmentation.\\\hline
			 
% 			 \cite{xu2021improved}&Segmentation&\makecell{DIOR \cite{li2020object} \\HRRSD\cite{zhang2019hierarchical} \\ NWPU VHR-10 \cite{cheng2016learning}}&\makecell{AP \\ FPS \\ AR_s \\ IoU}&Introduces the MRS-1800 remote sensing mask dataset, proposed a swin transformer based profiting from the both transformers and CNNs advantages, and designed a local perception Swin transformer backbone.\\\hline
			 
% 			 \cite{panboonyuen2021transformer}&Segmentation &\makecell{Vaihingen\cite{rottensteinerinternational} \\Thailand North Landsat-8 corpus (private) \\ Thailand Isan Landsat-8 corpus (private)}&\makecell{F1 \\ Precision \\ Recall \\ IoU \\ Accuracy}&An alternative perspective for semantic segmentation via prefacing decoder designs for transformer models.\\\hline
			 
% 			 \cite{xu2021efficient}&Segmentation &\makecell{Potsdam \cite{isprs20192d} \\Vaihingen\cite{rottensteinerinternational}}&\makecell{F1 \\ Precision \\ Recall \\ mIoU \\ Accuracy \\ OA}&A novel transformer model to realize lightweight edge classification.\\\hline
			 
% %--------------------------------------------------------
% 			 \cite{chen2021building}&Building Extraction &\makecell{WHU \cite{ji2018fully} \\INRIA\cite{maggiori2017can}}&\makecell{IoU\\OA\\F1}&Introduced  a dual pathway transformer for capturing the channel and spatial direction long range dependences\\\hline
			 
% 			 \cite{xiao2022swin}&Building Extraction &\makecell{WHU \cite{ji2018fully} \\Massachusetts\cite{maggiori2017can}}&\makecell{IoU\\F1}&introduced swim transformer based encoding framework named as STEB-UNet\\\hline
			 
% 			 \cite{wang2022buildformer}&Building Extraction &\makecell{WHU \cite{ji2018fully} \\Massachusetts\cite{maggiori2017can}
% 			 \\INRIA\cite{maggiori2017can}}&\makecell{IoU\\F1\\ Precision \\ Recall }&introduced swim transformer based framework named as BuildFormer, which consist of window based linear attention\\\hline
			 
% 			 \cite{qiu2022transferring}&Building Extraction &\makecell{Massachusetts\cite{maggiori2017can}
% 			 \\INRIA\cite{maggiori2017can}}&\makecell{IoU\\F1\\ Precision \\ Recall }&Explore the generalizability of building extraction models to different sub areas. \\\hline
% 			 %-------------------------------------------------%
% 		    \cite{shen2020remote}&\makecell{Image Captioning} &\makecell{RSICD\cite{lu2017exploring} \\UCM-captions \cite{yang2010bag,qu2016deep}\\Sydney-Caption\cite{zhang2014saliency,qu2016deep}}
% 			&\makecell{BLEU\\ROUGE\\METEOR\\CIDEr}&Presents a novel transformer based and reinforcement learning model.\\\hline
			
% 			MLAT\cite{liu2022remote}&\makecell{Image Captioning} &\makecell{RSICD\cite{lu2017exploring} \\UCM-captions \cite{yang2010bag,qu2016deep}\\Sydney-Caption\cite{zhang2014saliency,qu2016deep}}
% 			&\makecell{BLEU\\ROUGE_L\\METEOR\\CIDEr}&Introduced an encoder-decoder architecture.\\\hline
			
% 			\cite{Ren22RS}&\makecell{Image Captioning} &\makecell{RSICD\cite{lu2017exploring} \\UCM-captions \cite{yang2010bag,qu2016deep}\\Sydney-Caption\cite{zhang2014saliency,qu2016deep}}
% 			&\makecell{BLEU\\ROUGE\\METEOR\\CIDEr}&Introduces a topic token-based mask transformer framework.\\\hline
			
% 			\cite{Ren22RS}&\makecell{Image Captioning} &\makecell{RSICD\cite{lu2017exploring} \\UCM-captions \cite{yang2010bag,qu2016deep}\\Sydney-Caption\cite{zhang2014saliency,qu2016deep}}
% 			&\makecell{BLEU\\ROUGE\\METEOR\\CIDEr\\Self-CIDEr}&Introduces a transformer-based multi-stage enhancement structure.\\\hline
% 			%-------------------------------------------------%
% 			TR-MISR\cite{an2022tr}&\makecell{Image Super Resolution}&\makecell{RSICD\cite{lu2017exploring} \\UCM-captions \cite{yang2010bag,qu2016deep}\\PROBA-V\cite{martens2019super}}
% 			&\makecell{cPSNR\\cSSIM}&Investigates the multiimage super-resolution problem, a transformer-based approach is introduced comprised of three parts.\\\hline
% 			%-------------------------------------------------%
% 			%MSNet\cite{li2021msnet}&\makecell{Spatiotemporal Fusion}&\makecell{Aluhorqin Banner\cite{emelyanova2013assessing}\\Lower Gwydir Basin\cite{emelyanova2013assessing}\\Coleambally Irrigation District\cite{emelyanova2013assessing}}
% 			%&\makecell{SAM\\RMSE\\ERGAS\\SSIM\\CC\\MSE\\PSNR}&Introduced a transformer and convolution based network for remote sensing spatiotemporal fusion.\\\hline

%             %SwinSTFM\cite{chen2022swinstfm}&\makecell{Spatiotemporal Fusion}&\makecell{Aluhorqin Banner\cite{emelyanova2013assessing}\\Lower Gwydir Basin\cite{emelyanova2013assessing}\\Coleambally Irrigation District\cite{emelyanova2013assessing}}
% 			%&\makecell{{SAM\\RMSE\\ERGAS\\SSIM\\CC\\UIQI}}&Presents a novel swin transformer and linear spectral mixing theory based.\\\hline
			
% 			%MSFusion\cite{yang2022msfusion}&\makecell{Spatiotemporal Fusion}&\makecell{colembaly irrigation area\cite{emelyanova2013assessing}\\Lower Gwydir Basin\cite{emelyanova2013assessing}\\Daxing\cite{li2020spatio}}
% 			%&\makecell{{SAM\\RMSE\\ERGAS\\SSIM\\CC}}&Illustrated a texture transformer and CNN based model.\\\hline
			

% 		\end{tabular}
% 		}\caption{An overview of transformers-based approaches in VHR remote sensing imaging. Here, we highlight methods for different VHR remote sensing tasks.  }
% 	\label{tab:Main_table}}
% \end{table*}

\begin{table*}[t!]
 \renewcommand{\arraystretch}{1.5}
 	\centering
 	{\resizebox*{\textwidth}{\textheight}{%
 	%\resizebox{!}{.40\paperheight}{%
 	%\resizebox{\textwidth}{!}{
 	%\begin{longtable}{|*{3}{>{\centering\arraybackslash}p{3cm}|}}
 	\begin{tabular}{V{3}l|c|c|c|P{7cm}V{3}} \hlineB{3}
		
 		\rowcolor{mygray}	\textbf{Method}& \textbf{Task}& \textbf{Datasets}& \textbf{Metrics}& \textbf{Highlights} \\\hlineB{2}
			
			
			MSPSNet \cite{guo2021deep}&Change Detection &\makecell{SYSU-CD\cite{shi2021deeply},\\ LEVIR\cite{chen2020spatial}}	&\makecell{F1 score}&Introduces a multi-scale Siamese framework employing a parallel convolutional structure for feature integration of different temporal images and self-attention for feature refinement. \\\hline
			
			SwinSUNet \cite{zhang2022swinsunet}&Change Detection &\makecell{CCD\cite{lebedev2018change},\\ WHU\cite{ji2018fully},\\ OSCD\cite{daudt2018urban},\\ HRSCD\cite{daudt2019multitask}}
			&\makecell{F1 score}&Introduces a Swin transformer-based network with a Siamese U-shaped structure having encoder, fusion and decoder modules.\\\hline
			
            TransUNetCD \cite{li2022transunetcd}&Change Detection &\makecell{WHU\cite{ji2018fully},\\ LEVIR\cite{chen2020spatial},\\ CCD\cite{lebedev2018change},\\ DSIFN\cite{zhang2020deeply}, \\OSCD\cite{daudt2018urban},\\ S2Looking\cite{shen2021s2looking}}
			&\makecell{F1 score}&Introduces a framework integrating merits of transformers and UNet through capturing enriched contextualized features which are upsampled and fused with multi-scale features to generate global-local features. \\\hline
			
			Hybrid-TransCD \cite{HybridTransCD}&Change Detection &\makecell{LEVIR\cite{chen2020spatial},\\ SYSU-CD\cite{shi2021deeply}}
			&\makecell{F1 score}&Introduces a multi-scale transformer that encodes both fine-grained and large object features through heterogeneous tokens via multiple receptive fields.\\\hline
			
			
%----------------------------------------------------------------%
			 CCTNet \cite{wang2022cctnet}&Segmentation &\makecell{Barley Remote Sensing Dataset \cite{barley}}&\makecell{F1 score,\\ Overall accuracy}& Proposes a hybrid CNN-transformers framework to combine local details and global conextual information for crop segmentation. \\\hline
			 
			 STransFuse \cite{9573374}&Segmentation &\makecell{Potsdam\cite{Potsdam},\\ Vaihingen\cite{Vaihingen}}&\makecell{F1 score,\\ Overall accuracy}& Introduces a framework that encodes both coarse-grained as well as fine-grained features at multiple scales which are fused using self-attentive mechanism. \\\hline
			 
			 Trans-CNN \cite{9686732}&Segmentation&\makecell{Potsdam\cite{Potsdam},\\ Vaihingen\cite{Vaihingen}}&\makecell{F1 score,\\ Overall accuracy}& Introduces a framework with a Swin transformer backbone to capture long-range dependencies and a U-shaped decoder with depth-wise separable convolution to encode local details. \\\hline
			 
			% Xu \etal\cite{xu2021improved}&Segmentation&\makecell{DIOR\cite{li2020object}, HRRSD\cite{zhang2019hierarchical},  NWPU VHR-10\cite{cheng2016learning}}&\makecell{F1 score, Overall accuracy}&A local perception Swin transformer backbone, taking advantage of both CNNs and transformers.\\\hline
			 
		SwinTF \cite{panboonyuen2021transformer}&Segmentation &\makecell{Vaihingen\cite{Vaihingen},\\ Thailand North Landsat-8 corpus (private),\\ Thailand Isan Landsat-8 corpus (private)}&\makecell{F1 score,\\ Overall accuracy}&Introduces a framework with pre-trained Swin backbone along with a U-Net, feature pyramid network and a pyramid scene parsing network for segmentation. 
\\\hline
			 
			Efficient-T \cite{xu2021efficient}&Segmentation &\makecell{Potsdam\cite{Potsdam},\\ Vaihingen\cite{Vaihingen} }&\makecell{F1 score,\\ Overall accuracy}& Proposes a light-weight framework consisting of an implicit edge enhancement scheme along with a Swin transformers.\\\hline
			%---------

            STT \cite{chen2021building}&Building Extraction &\makecell{WHU\cite{ji2018fully},\\ INRIA\cite{maggiori2017can}}&\makecell{IoU,\\ Overall accuracy,\\ F1 score}&Introduces a transformers framework to learn long-range dependencies both in the spatial and channel direction. \\\hline
			 
			 STEB-UNet \cite{xiao2022swin}&Building Extraction &\makecell{WHU\cite{ji2018fully},\\ Massachusetts\cite{maggiori2017can}}&\makecell{IoU,\\ F1 score}&Introduces a transformers framework capturing semantic information from multi-scale features which are further fused to local features. \\\hline
			 
			 BuildFormer \cite{wang2022buildformer}&Building Extraction &\makecell{WHU\cite{ji2018fully},\\ Massachusetts\cite{maggiori2017can},\\
			 INRIA\cite{maggiori2017can}}& \makecell{IoU,\\ F1 score}& Introduces an architecture consisitng of a window-based linear attention and a convolutional MLP.\\\hline
			 
			 T-Trans \cite{qiu2022transferring}&Building Extraction &\makecell{Massachusetts\cite{maggiori2017can}\\
			 ,INRIA\cite{maggiori2017can}}&\makecell{IoU,\\ F1 score}& Explores the task of generalizability of building extraction models to different areas and introduces a transfer learning method to fine-tune models from one area to a subset of another unseen area.  \\\hline
			 
 %-------------------------------------------------%
 
		    TRL \cite{shen2020remote}&\makecell{Image Captioning} &\makecell{RSICD\cite{lu2017exploring},\\ UCM-captions \cite{UCMCaptions},\\ Sydney-Caption\cite{sydney}}
			&\makecell{BLEU,\\ ROUGE,\\ METEOR,\\ CIDEr}&Proposes an approach adapting transformers by integrating residual connections, dropout and adatpive feature fusion for remote sensing image caption generation. \\\hline
			
			MLAT\cite{liu2022remote}&\makecell{Image Captioning} &\makecell{RSICD\cite{lu2017exploring},\\ UCM-captions\cite{UCMCaptions},\\ Sydney-Caption\cite{sydney}]}
			&\makecell{BLEU,\\ ROUGE,\\ METEOR,\\ CIDEr}&Introduces an architecture where multi-scale features from CNN layers are extracted in encoder and a multi-layer aggregated transformer in the decoder uses those features for sentence generation. \\\hline
			
			Ren \etal\cite{ren2022mask}&\makecell{Image Captioning} &\makecell{RSICD\cite{lu2017exploring},\\ UCM-captions\cite{UCMCaptions},\\ Sydney-Caption\cite{sydney}}
			&\makecell{BLEU,\\ ROUGE,\\ METEOR,\\ CIDEr}&Proposes a topic token-based mask transformers  with the topic token being integrated into encoder while serving as prior in decoder for capturing global semantic relationships.\\\hline
			
% 			\cite{Ren22RS}&\makecell{Image Captioning} &\makecell{RSICD\cite{lu2017exploring} \\UCM-captions \cite{yang2010bag,qu2016deep}\\Sydney-Caption\cite{zhang2014saliency,qu2016deep}}
% 			&\makecell{BLEU\\ROUGE\\METEOR\\CIDEr\\Self-CIDEr}&Introduces a transformer-based multi-stage enhancement structure.\\\hline

%-------------------------------------------------%
			TR-MISR \cite{an2022tr}&\makecell{Image Super Resolution}&\makecell{RSICD\cite{lu2017exploring},\\ UCM-captions\cite{UCMCaptions},\\ PROBA-V\cite{martens2019super}}
			&\makecell{cPSNR,\\ cSSIM}&Introduces a transformers-based architecture with an encoder having residual blocks, a fusion module along with a super-pixel convolution-based decoder for multi-image super-resolution. \\\hline
			
			MSE-Net \cite{lei2021transformer}&\makecell{Image Super Resolution}&\makecell{UCMerced\cite{ucmerced},\\ AID\cite{xia2017aid}}
			&\makecell{cPSNR,\\ cSSIM}&Proposes a multi-stage enchancement framework to utilize features from different stages and further integrating them with standard super-resolution technique for combining multi-resolution low as well as high-dimension feature representations. \\\hline
			
		SRT \cite{ye2021super}&\makecell{Image Super Resolution}&\makecell{UCMerced\cite{ucmerced}}
			&\makecell{cPSNR,\\ cSSIM}&Introduces a hybrid framework that integrates local features from CNNs and global features from transformers. \\\hline			 
			 
			 
 %-------------------------------------------------%
 		\end{tabular}}
 		
 	}
 	
\end{table*}

==> Transformers in remote sensing-a survey/Table2.tex <==
%\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

%\usepackage{lscape}

%\begin{landscape}
%\begin{table}[h]
\begin{table*}
%\renewcommand{\arraystretch}{1.5}
	\centering
	%\Large
		\caption{Overview of transformers-based approaches in Hyperspectral imaging. Here, we highlight methods for different Hyperspectral remote sensing tasks.} \label{tab:HSISAR}%}
	%{\resizebox*{\textwidth}{\textheight}{%
	%\resizebox{!}{.40\paperheight}{%
	\resizebox{\textwidth}{!}{
	%\begin{longtable}{|*{3}{>{\centering\arraybackslash}p{3cm}|}}
	\begin{tabular}{V{3}l|c|c|c|P{7cm}V{3}} \hlineB{3}
		\rowcolor{mygray} \multicolumn{5}{|c|}{\textbf{Transformers in Hyperspectral Imagery}} \\ \hlineB{2}
		\rowcolor{mygray}	\textbf{Method}& \textbf{Task}& \textbf{Datasets}& \textbf{Metrics}& \textbf{Highlights} \\\hlineB{2}
			
			%---------


            
			 SpectralFormer \cite{hong2021spectralformer} & Classification&\makecell{Indian Pines\cite{indian},\\ Pavia University\cite{pavia},\\ {Houston2013}\cite{houston}}&\makecell{Overall classification accuracy,\\ Kappa}&  Introduces a transformers-based backbone to capture spectrally local information from nearby hyperspectral bands by generating group-wise spectral embeddings.
\\\hline
			 
			 MCT \cite{jia2022multiscale} &Classification&\makecell{Salinas\cite{salinas},\\ Yellow River Estuary}&\makecell{Overall classification accuracy,\\ Kappa}& Proposes a multi-scale convolutional transformer to encode spatial-spectral information that is integrated with transformers network.\\\hline
			 
			 MFT\cite{roy2022multimodal}&Classification&\makecell{University of Houston\cite{houston},\\ Trento,\\ MUUFL Gulfport\cite{gader2013muufl},\\ Augsburg scenes}&\makecell{Overall classification accuracy,\\ Kappa}& Proposes a multi-modal transfomers that derives class tokens from multi-modal data along with the standard hyperspectral patch tokens.
\\\hline
 
 			 CTN \cite{zhao2022convolutional} &Classification&\makecell{Indian Pines\cite{indian},\\ Pavia University\cite{pavia}}&\makecell{Overall classification accuracy,\\ Kappa}&  Introduces a convolutional transformer network with dedicated blocks that integrates local and global features from hyspectral image patches.\\\hline
			 
			 DHViT \cite{xue2022deep} &Classification&\makecell{Trento,\\ Houston 2013\cite{houston},\\ Houston 2018\cite{Houston18}}&\makecell{Overall classification accuracy,\\ Kappa}& Introduces an approach comprising a spectral sequence transformer to encode features along the spectral dimension and a spatial hierarchical transformer to produce hierarchical spatial features for hyperspectral and LiDAR data. \\\hline
			 
			 DSS-TRM \cite{liu2022dss}&Classification&\makecell{Pavia University\cite{pavia},\\ Salinas\cite{salinas},\\ Indian Pines\cite{indian}}&\makecell{Overall classification accuracy,\\ Kappa}& Introduces a transformers-based approach consisting of spectral self-attention  and spatial self-attention to capture interactions along spectral and spatial dimension, respectively. \\\hline
			 
 			 HiT \cite{yang2022hyperspectral}&Classification&\makecell{Indian Pines\cite{indian},\\ Pavia University\cite{pavia},\\ Houston2013\cite{houston},\\ Xiongan}&\makecell{Overall classification accuracy, Kappa}& Proposes a hyperspectral image transformer consisting of a 3D convolution projection module to encode local spatial-spectral details and a conv-permutator modue to capture the information along height, width and spectral dimensions. \\\hline
 
 			 HSI-BERT \cite{he2019hsi} &Classification&\makecell{Indian Pines\cite{indian},\\ Pavia University\cite{pavia},\\ Salinas\cite{salinas}}&\makecell{Overall classification accuracy}&  Proposes a transformers-based method that captures capture global dependencies using a bi-direction encoder representation. \\\hline
			 
			 SSFTT \cite{sun2022spectral} &Classification&\makecell{Indian Pines\cite{indian},\\ Pavia University\cite{pavia},\\ Houston 2013\cite{houston}}&\makecell{Overall classification accuracy,\\ Kappa}& Proposes a spectral–spatial feature tokenization transformer that utilizes both spectral-spatial shallow and semantic features for representation and learning. \\\hline
			 
			 SSTN \cite{zhong2021spectral}&Classification&\makecell{Pavia University\cite{pavia},\\ Kennedy Space Center,\\ Indian Pines\cite{indian},\\ University of Houston\cite{houston},\\ Pavia Center\cite{paviacenter}}&\makecell{Overall classification accuracy,\\ Kappa}& Introduces a spectral–spatial transformer with a spatial attention and a spectral association module. The two modules perform spectral and spatial association through the integration of spectral and spatial locations, respectively. \\\hline
			 
			 
%----------------------------------------------------------%			 
			 % Li \etal \cite{li2011hyperspectral}&Segmentation &\makecell{AVIRIS Indian Pines, ROSIS Pavia}&\makecell{OA}&A Supervised Bayesian approach is used along with active learning for HS segmentation.\\\hline
			 
			 % Yun \etal \cite{yun2021spectr}&Segmentation &\makecell{choledoch}
			 % &\makecell{DSC, IoU, Hausdor Distance}& The contextual feature learning along spectral bands is used to capture the wide range dependencies.\\\hline
            
			 % Mohan \etal \cite{mohan2007spatially}&Segmentation &\makecell{Indian Pines, EO-1 satellite}
			 % &\makecell{Euclidean, vector angle, $L_{1}$}& Invested the idea of how dimensional reduction aids in impacting segmentation and classification tasks.\\\hline
			 
			% Li \etal \cite{li2010semisupervised}&Segmentation &\makecell{Salinas, Indian Pines}
			% &\makecell{OA}& Semi supervised segmentation alogorithm is used for segmenting the high dimensional hyperspectral images.\\\hline
			 
			 			 
   %          Zhou \etal \cite{zhou2021swin}&Segmentation &\makecell{Choledoch}
			% &\makecell{mIoU, mDice, aAcc, kappa}& A swim-spectral transformer is used for segmentation of H.S. Image.\\\hline


%----------------------------------------------------------%
			% Shi \etal\cite{shi2020hyperspectral}&Detection&\makecell{Synthetic Data, San Diego, Avon, Indian Pines}
			% &\makecell{3D-ROC and 2D-ROC}&Introduces a network that reduces the overabundance of spectral and spatial concurrently.\\\hline

			% Rao \etal\cite{rao2022siamese}&Detection&\makecell{San Diego, Airport–Beach–Urban, Nuance Cri}
			% &\makecell{ROC, AUC, FAR, Separability Map}& A siamese network is introduced to address the drawback of similarity metric learning.\\\hline
			
			
%----------------------------------------------------------------%
			 CTIN \cite{zhou2022panformer}&Pan-Sharpening&\makecell{worldview II\cite{WVii},\\ worldview III\cite{wviii},\\ GaoFen-2}&\makecell{IQA,\\ ERGAS,\\ PSNR,\\ SAM}& A transformers-based approach is introduced, where multi-spectral and panchromatic features are captured for joint feature learning across modalities. Further, an invertible neural module performs feature fusion to generate pansharpened images. \\\hline
			 
			 HyperTransformer \cite{Bandaracvpr22}&Pan-Sharpening&\makecell{Pavia Center\cite{paviacenter},\\ Botswana\cite{Botswana},\\ Chikusei\cite{NYokoya2016}}&\makecell{Cross-correlation(CC),\\ Spectral Angle Mapping (SAM),\\ RSNR,\\ ERGAS,\\ PSNR}& Introduces a transformers-based framework with separate feature extractors for panchromatic and hyperspectral images and a spectral-spatial fusion module to learn cross-feature space dependencies of features. \\\hline
			 
			 PMACNet \cite{liang2022pmacnet}&Pan-Sharpening&\makecell{worldview II\cite{WVii},\\ worldview III\cite{wviii}}&\makecell{spatial correlation coefficient(SCC),\\ spectral angle mapper (SAM)}& Introduces a framework with a parallel CNN structure to learn ROIs from low-resolution image and residuals from high-resolution image. It also contains a a pixel-wise attention module to adapt residuals on the learned ROIs.\\\hline			 
			 
			 CPT-noRef \cite{li2022pan}&Pan-Sharpening&\makecell{Gaofen-1,\\ worldview II\cite{WVii},\\ Pleiades\cite{pleiades}}&\makecell{IQA,\\ ERGAS,\\ SAM,\\ correlation coefficient(CC)}& A CNN-transformers framework where global features are generated using transformers and local features are constructed using a shallow CNNs. The features are combined and a loss formulation having spatial and spectral losses are utilized for training.\\\hline
			 
			 MSIT \cite{zhang2022multiscale}&Pan-Sharpening&\makecell{GeoEye-1,\\ QuickBird\cite{QB}}&\makecell{ERGAS,\\ SAM,\\ Q4}& Introduces a multi-scale spatial–spectral interaction transformer with a convolution-transformer encoder for generating multi-scale global and local features from both low-resolution and panchromatic images.\\\hline			 
			 
			 Su \etal \cite{su2022transformer}&Pan-Sharpening&\makecell{worldview II\cite{WVii}, QuickBird\cite{QB}, GaoFen-2}&\makecell{spatial correlation coefficient(SCC),\\ ESGAS,\\ RMSE,\\ SAM,\\ Q4}& A transformers-based approach with spatial and spectral feature extraction performed using a Swin model. \\\hline			 
			 
			 
 %-------------------------------------------------%
 		\end{tabular}
 		}
 	
 	
\end{table*}
%\end{table}
 %\end{landscape}

==> Transformers in remote sensing-a survey/Table3.tex <==

\begin{table*}[h]
%\renewcommand{\arraystretch}{1.5}
	\centering
	\caption{Overview of transformers-based approaches in SAR imaging. Here, we highlight methods for different SAR remote sensing tasks.}
	%{\resizebox*{\textwidth}{\textheight}{%
	%\resizebox{!}{.40\paperheight}{%
	\resizebox{\textwidth}{!}{
	%\begin{longtable}{|*{3}{>{\centering\arraybackslash}p{3cm}|}}
	\begin{tabular}{V{3}l|c|c|c|P{7cm}V{3}} \hlineB{3}
		\rowcolor{mygray} \multicolumn{5}{|c|}{\textbf{Transformers in SAR Satellite Imagery}} \\ \hlineB{2}
		\rowcolor{mygray}	\textbf{Method}& \textbf{Task}& \textbf{Datasets}& \textbf{Metrics}& \textbf{Highlights} \\\hlineB{2}
			
			%---------



			 ViT-PolSAR \cite{9658539} &Classification&\makecell{AIRSAR Flevoland \cite{norikane1992application},\\ ESAR Oberpfaffenhofen\cite{ESAR},\\ AIRSAR San Francisco\cite{sanfran},\\ ALOS2 San Francisco\cite{alos2}}&\makecell{AA,\\ OA,\\ Kappa}& Explores transformers, where self-attention is used to capture long-range dependencies followed by MLP for polarimetric SAR image classification.\\\hline
			 
			 GLNS \cite{9713848} &Classification&\makecell{Gaofen-3 SAR\cite{Gaofen3},\\ F-SAR\cite{FSAR}}&\makecell{AA,\\ OA,\\ Kappa}&Introduces a global–local network structure to exploit the merits of CNNs and transformers with local and global features that are fused to perform classification. \\\hline
			 
			 ST-PN \cite{cai2022st}&Classification&\makecell{MSTAR\cite{MSTAR}}&\makecell{Accuracy}&Proposes a spatial transformer network for spatial alignment of features extracted from CNNs for few-shot SAR classification. 

\\\hline
			 
			 
			 
			 
%----------------------------------------------------------%			 
			 GCBANet \cite{ke2022gcbanet}&Segmentation &\makecell{SSDD\cite{8124934},\\ HRSID\cite{9127939}}&\makecell{AP}&Introduces a transformers-based approach with a global contextual block for capturing spatial holistic long-range dependencies and a boundary-aware prediction scheme for estimating the boundaries of ship. \\\hline
			 
			 CRTransSar \cite{xia2022crtranssar}&Detection &\makecell{SMCDD\cite{xia2022crtranssar},\\ SSDD\cite{8124934}}
			 &\makecell{Accuracy,\\ Recall,\\ mAP,\\ F1}& Proposes a backbone based on convolutional and attention blocks for capturing both local and global features.\\\hline
            
			 Geospatial Transformers \cite{chen2022geospatial}&Detection &\makecell{Gaofen-3\cite{Gaofen3}}
			 &\makecell{DR,\\ FAR}& 
Introduces a framework with multi-scale geo-spatial attention for aircraft detection in SAR imaging. \\\hline
			 
			SFRE-Net \cite{zhang2022sfre}&Detection &\makecell{Gaofen-3\cite{Gaofen3}}
			&\makecell{Precision,\\ Recall,\\ F1}& Introduces a feature relation enhancement architecture consisting of a fusion pyramid structure and a context attention enhancement technique. \\\hline
			 
			 			 
            3DET-ViT \cite{ma2021end}&Detection &\makecell{L1B SAR\cite{L1B}}
			&\makecell{AP,\\ AR,\\ Mean Offset}&
Proposes a transformers-based framework that takes incidence angle as a prior token with a feature description operator employing scattering centers for prediction refinement. 
\\\hline


%----------------------------------------------------------%
			ID-ViT \cite{Perera22neural}&Despeckling&\makecell{Berkeley Segmentation Dataset\cite{937655}}
			&\makecell{PSNR,\\ SSIM}& Proposes a framework comprising an encoder to learn global dependencies among SAR image regions, where the network is trained using synthetic speckled data. 
\\\hline
			
			
%----------------------------------------------------------------%
			 CLT \cite{Huihui22neural}&Change Detection &\makecell{Brazil and Namibia datasets\cite{BrazilNamibia},\\ simulation data\cite{Huihui22neural}}&\makecell{KC}& 
Introduces a self-supervised contrastive representation learning method with a convolution-enhanced transformer to generate hierarchical representations for distinguishing changes from HR SAR images. \\\hline
			 
%--------------------------------------------------------
			 CF-ViT \cite{Fan22RS}&Image Registration&\makecell{MegaDepth\cite{MegaDepthLi18}}&\makecell{KC}& A CNN-transformers framework that first performs coarse registration on the down-sampled image, followed by registration of image pairs via a CNN-transformer module with the resulting point pair subsets integrated to obtain final global registration. \\\hline
			 
 %-------------------------------------------------%
 		\end{tabular}
 		}
 	%	\caption{An overview of transformers-based approaches in SAR remote sensing imaging. Here, we highlight methods for different SAR remote sensing tasks.}
 	\label{tab:SAR}%}
\end{table*}
